Defect-like structures and localized patterns in SH357

We study numerically the cubic-quintic-septic Swift-Hohenberg (SH357) equation on bounded one-dimensional domains. Under appropriate conditions stripes with wave number $k\approx 1$ bifurcate supercritically from the zero state and form S-shaped branches resulting in bistability between small and large amplitude stripes. Within this bistability range we find stationary heteroclinic connections or fronts between small and large amplitude stripes, and demonstrate that the associated spatially localized defect-like structures either snake or fall on isolas. In other parameter regimes we also find heteroclinic connections to spatially homogeneous states, and a multitude of dynamically stable steady states consisting of patches of small and large amplitude stripes with different wave numbers or of spatially homogeneous patches. The SH357 equation is thus extremely rich in the types of patterns it exhibits. Some of the features of the bifurcation diagrams obtained by numerical continuation can be understood using a conserved quantity, the spatial Hamiltonian of the system.

==> fig0pre.tex <==
%\begin{widetext}
 \begin{figure*}%[H]%[htpb]
\begin{tabular}{p{0.48\twi}p{5mm}p{0.48\twi}}
{\small (a) $a{=}2$: BD of $\up$ (black), $\uhl$ (blue) and one snaking branch (red) 
of fronts between $\upl$ and $u=0$ (left folds) and $\uplg$ and $\upsg$ 
(right folds), respectively} &&{\small (b) $a{=}5$: BD of $\up$ (black), $\uh$ (blue) and one snaking branch (red) of localized $\uplg$ over $\upsg$ patterns} \\
\ig[width=0.15\twi,height=36mm]{2-L2}
\hs{-1mm}\raisebox{16mm}{\begin{tabular}{l}
\ig[width=0.17\twi,height=16mm]{2-fp10}\\
\ig[width=0.17\twi,height=16mm]{2-fp11}
\end{tabular}}
\ig[width=0.14\twi,height=36mm]{2-H}
&&
\ig[width=0.15\twi,height=36mm]{5-L2r}
\hs{-2mm}\raisebox{16mm}{\begin{tabular}{l}
\ig[width=0.17\twi,height=16mm]{5-50}\\
\ig[width=0.17\twi,height=16mm]{5-200}
\end{tabular}}
\ig[width=0.14\twi,height=36mm]{5-H}
\\[-1mm]
\end{tabular}
\begin{tabular}{p{0.98\twi}}
{\small (c) $a{=}9.5$: BD for $\up$ and $\uh$ with zoom showing two isolas (magenta, blue) and 
a branch of solutions involving $\pm\uhl$ (red), with sample solutions}\\ 
\ig[width=0.15\twi,height=45mm]{l2-9-5}
\ig[width=0.22\twi,height=45mm]{9-5-L2dr}
\hs{-1mm}\raisebox{20mm}{\begin{tabular}{l}
\ig[width=0.2\twi]{n25}\ig[width=0.2\twi]{n100}\\
\ig[width=0.2\twi]{n125}\ig[width=0.2\twi]{n200}\\
\ig[width=0.2\twi,height=15mm]{9-li1-1}\ig[width=0.2\twi,height=15mm]{9-li2-1}
\end{tabular}}
\hs{-4mm}\ig[width=0.16\twi,height=45mm]{h9-5}
\end{tabular}
\vs{-2mm}
   \caption{{\small Solutions of % Equation 
\reff{sh2} on $\Om=(-10\pi,10\pi)$. (a) $a=2$: for $\lam<0$ there is bistability of $\upl$ with $u=0$, for $\lam>0$ bistability 
of $\upl$ and $\ups$ and the snake may straddle $\lam=0$. 
(b) $a=5$: ``classical'' snaking of heteroclinic cycles 
between $\upsg$ and $\uplg$. (c) $a=9.5$: breakup of classical snaking into stacks of isolas, and heteroclinic cycles to the $k=0$ branch. The right panel in each case shows self-intersections of the spatial Hamiltonian $H(\cdot)$ corresponding to different types of Maxwell points.
%At $a=9.5$ there are multiple intersections of all these branches. 
See Remark \ref{rem1}(d) for the 
naming and plotting conventions in these and the following plots.
\label{f0}}}
\end{figure*}
%\end{widetext}


==> fig3pre.tex <==
\begin{figure}[H]
\bce 
\begin{tabular}{ll}
(a)&(b)\\
\ig[width=0.2\twi,height=40mm]{5-H}&
\ig[width=0.17\twi,height=40mm]{5-L2}\\
(c)&(d)\\
\hs{-0mm}\ig[width=0.22\twi,height=45mm]{5-L2b}&
\hs{-2mm}\raisebox{22mm}{
\begin{tabular}{l}
\ig[width=0.22\twi,height=13mm]{5-50}\\
\ig[width=0.22\twi,height=13mm]{r7-0}\\
\ig[width=0.22\twi,height=13mm]{5-l2-100b}
\end{tabular}}
\end{tabular}\\[-0mm]
\begin{tabular}{l}
(e)\\
\ig[width=0.22\twi,height=13mm]{r7-10}
\ig[width=0.22\twi,height=13mm]{r7-bp1}\\
\hs{-0mm}\ig[width=0.22\twi,height=13mm]{5-ol-fpt3}
\ig[width=0.22\twi,height=13mm]{5-h25}
\end{tabular}\\[-2mm]
\ece
\vs{-2mm}
   \caption{{\small %Equation \reff{sh1} with $f(u)$ as in \reff{sh2}--\reff{bsel} and 
$a=5$. (a) $H$ on the first four branches of periodic solutions (black to light grey), %$k=1,\ldots$, 
and the homogeneous solution $\uh$ ($k=0$, blue). (b) $\|u\|$ for the
primary periodic branch (black) and for $\uh$ (blue), together with a snake (red) of cycles between $\upsg$ and $\uplg$, consisting of even solutions, and a pattern branch between two Turing bifurcations on $\uhl$ (magenta). (c) Zoom of the snake, together with two rungs (brown) that connect the even snake and the odd snake (blue). (d) Even solutions (close to left folds) corresponding to (c).  (e) Sample solutions from the light brown rung and the odd parity snake (blue branch) in (c), and from the magenta branch ({\tt hom2hom}) in (b). 
  \label{f1}}}
\end{figure}


==> fig5pre.tex <==
\begin{figure*}[htbp]
\bce 
\begin{tabular}{lll}
(a)&(b)&(c)\\
\ig[width=0.25\twi,height=80mm]{lBD3}&
\hs{-3mm}\raisebox{40mm}{
\begin{tabular}{l}
\ig[width=0.4\twi,height=18mm]{l135}\\
\ig[width=0.4\twi,height=18mm]{l1027}\\
\ig[width=0.4\twi,height=18mm]{fp25}\\
\ig[width=0.4\twi,height=18mm]{fp17}\\
\end{tabular}}&
\hs{-3mm}\raisebox{40mm}{
\begin{tabular}{l}
\ig[width=0.2\twi,height=19mm]{135f}\\
\ig[width=0.2\twi,height=19mm]{1027f}\\
\ig[width=0.2\twi,height=19mm]{fp25f}\\
\ig[width=0.2\twi,height=19mm]{fp17f}
\end{tabular}}
\end{tabular}\\
\begin{tabular}{lll}
(d)&(e)&(f)\\
\ig[width=0.25\twi,height=45mm]{lBD3b}&
\hs{-3mm}\raisebox{25mm}{
\begin{tabular}{l}
\ig[width=0.40\twi,height=18mm]{6741}\\
\ig[width=0.40\twi,height=18mm]{7388}
\end{tabular}}&
\hs{-0mm}\raisebox{5mm}{\ig[width=0.23\twi]{lf2}}
\end{tabular}
\ece
\vs{-7mm}
   \caption{{\small 
(a) Details of the $\uplg-\upsg-\uplg$ snake from Fig.~\ref{fl1}. (b,c) Sample solutions and Fourier transform.  (d,e) Left end of the 
snake and sample solutions. (f) Wave numbers of $\upsg$ (red) and $\uplg$ (blue) 
from the snake. \label{fl2}}}
\end{figure*}


==> fig6bpre.tex <==
\begin{figure}[htpb]
\bce 
\begin{tabular}{l}
(a)\\
\ig[width=0.25\twi,height=50mm]{i1z}\\
(b)\\
\hs{-0mm}\raisebox{0mm}{\begin{tabular}{l}
\ig[width=0.21\twi,height=14mm]{9-li1-1}\ig[width=0.21\twi,height=14mm]{ir2-7}\\
\ig[width=0.21\twi,height=14mm]{9-li1-72}\ig[width=0.21\twi,height=14mm]{ir2-24}\\
\ig[width=0.21\twi,height=14mm]{9-li1-108}\ig[width=0.21\twi,height=14mm]{ir2-46}\\
\ig[width=0.21\twi,height=14mm]{9-li1-134}\ig[width=0.21\twi,height=14mm]{9-li2-1}
\end{tabular}}
\end{tabular}
\ece
\vs{-2mm}
   \caption{{\small  (a) Zoom of the 
blue isola in Fig.~\ref{f3}(c) and associated rung structure. The labels ptnr,$i$ 
indicate stability properties with $i$ specifying the number of unstable
eigenvalues. (b) Sample solutions from (a).  \label{f3b}}}
\end{figure}


==> fig6pre.tex <==
\begin{figure}[htpb]
\bce 
\begin{tabular}{lll}
(a)&(b)&(c)\\
\hs{-2mm}\ig[width=0.16\twi,height=58mm]{h9-5}&
\hs{-2mm}\ig[width=0.12\twi,height=58mm]{l2-9-5}&
\hs{-1mm}\ig[width=0.19\twi,height=60mm]{9-5-L2d}
\end{tabular}\\
\begin{tabular}{l}
(d)\\
\ig[width=0.22\twi,height=14mm]{n25}\ig[width=0.22\twi,height=14mm]{n100}\\
\ig[width=0.22\twi,height=14mm]{n125}\ig[width=0.22\twi,height=14mm]{n200}\\
\ig[width=0.22\twi,height=14mm]{n250}\ig[width=0.22\twi,height=14mm]{n300}\\
\ig[width=0.22\twi,height=14mm]{n350}\ig[width=0.22\twi,height=14mm]{n400}
\end{tabular}
\ece
\vs{-2mm}
   \caption{{\small 
$a{=}9.5$, $\Om{=}(-10\pi,10\pi)$. (a) $H$ for solution branches plotted as in Fig.~\ref{f1}(a); there are now multiple intersections near $\lam=3.5$. (b) 
$\|u\|$ for the $k{=}1$ and $k{=}0$ branches, illustrating the multistability near $\lam=3.5$. (c) Two isolas of cycles between $\ups$ and 
$\upl$ obtained from suitable initial guesses, further discussed in Fig.~\ref{f3b}, and a branch (red) of 
$\upl$--$\ups$ cycles which passes near $\lam{=}3.5$ close to $\pm\uhl$. 
(d) Sample solutions from the red branch in (c).  \label{f3}}}
\end{figure}


==> fig7cpre2.tex <==
\begin{figure}[htpb]
\bce 
\begin{tabular}{l}
(a) $(a,\lam)=(5,1.3)$ \\
\ig[width=0.4\twi,height=20mm]{tpics/t2a}\\
%&\ig[width=0.4\twi,height=22mm]{tpics/t2b}\\
(b) $(a,\lam=(5,1.49)$\\
\ig[width=0.4\twi,height=20mm]{tpics/t11a}\\
 (c) $(a,\lam)=(5,1.5)$\\
\ig[width=0.4\twi,height=20mm]{tpics/t8a}\\
(d) $(a,\lam)=(5,1.3)$\\
\ig[width=0.4\twi,height=20mm]{tpics/t6a}\\
(e) $(a,\lam)=(9.5,3)$\\
\ig[width=0.4\twi,height=20mm]{tpics/t3a}\\
\end{tabular}
\ece
\vs{-2mm}
\caption{{\small Time evolution on $\Om=(-25\pi,25\pi)$ (a,d,e) and $\Om=(-40\pi,40\pi)$ 
    (b,c) in the form of space-time diagrams. Horizontal axis shows space $x$, vertical axis
    time $t$, %with a 3D plot in the right panel of (a). 
parameters as indicated.
Initial conditions consist of smooth amplitude and wavenumber transition between one state on the left and a different state on the right (the precise form appears not to matter provided it is not too gradual) and are given by  
(a) $u_0=1.5\cos(x)$ for $x<-9\pi$, $u_0(x)=0.5\cos(0.6x)$ for $x\ge -5\pi$; 
(b,c) $u_0=1.5\cos(x)$ for $x<-34\pi$, $u_0(x)=0.5\cos(0.6x)$ for $x\ge -28\pi$; 
(d) $u_0=1.5\cos(0.8x)$ for $x<-4\pi$, $u_0(x)=0.5\cos(x)$ for $x\ge 0$;
(e) $u_0=0$ for $x<-10\pi$, $u_0=2$ for $x\ge -10\pi$.
\label{f7}}}
\end{figure}


==> fig7cpre3.tex <==
\begin{figure*}[htpb]
\bce 
\begin{tabular}{lll}
(a1) $(a,\lam)=(5,1.3)$&(b) $(a,\lam=(5,1.49)$&(d) $(a,\lam)=(5,1.3)$\\ 
\ig[width=0.32\twi,height=20mm]{t2a}&
\ig[width=0.32\twi,height=20mm]{t11a}&
\ig[width=0.32\twi,height=20mm]{t6a}\\
(a2) same as (a1) as 3D plot&(c) $(a,\lam)=(5,1.5)$&(e) $(a,\lam)=(9.5,3)$\\
\ig[width=0.32\twi,height=22mm]{t2b}&
\ig[width=0.32\twi,height=20mm]{t8a}&
\ig[width=0.32\twi,height=20mm]{t3a}\\
\end{tabular}
\ece
\vs{-2mm}
\caption{{\small Time evolution on $\Om=(-25\pi,25\pi)$ (a,d,e) and $\Om=(-40\pi,40\pi)$ 
    (b,c) in the form of space-time diagrams. Horizontal axis shows space $x$, vertical axis
    time $t$, %with a 3D plot in the right panel of (a). 
parameters as indicated.
Initial conditions consist of smooth amplitude and wavenumber transition between one state on the left and a different state on the right (the precise form appears not to matter provided it is not too gradual) and are given by  
(a) $u_0=1.5\cos(x)$ for $x<-9\pi$, $u_0(x)=0.5\cos(0.6x)$ for $x\ge -5\pi$; 
(b,c) $u_0=1.5\cos(x)$ for $x<-34\pi$, $u_0(x)=0.5\cos(0.6x)$ for $x\ge -28\pi$; 
(d) $u_0=1.5\cos(0.8x)$ for $x<-4\pi$, $u_0(x)=0.5\cos(x)$ for $x\ge 0$;
(e) $u_0=0$ for $x<-10\pi$, $u_0=2$ for $x\ge -10\pi$.
\label{f7}}}
\end{figure*}


==> hudef.tex <==
\def\bexe{\begin{exercise}}\def\eexe{\eex\end{exercise}}
\def\bsol{\begin{solution}}\def\esol{\eex\end{solution}}
\def\bexa{\begin{example}}\def\eexa{\end{example}}
\def\brem{\begin{remark}}\def\erem{\end{remark}}
\def\bthm{\begin{theorem}}\def\ethm{\end{theorem}}
\def\blem{\begin{lemma}}\def\elem{\end{lemma}}
\def\bcor{\begin{corollary}}\def\ecor{\end{corollary}}
\def\bdefi{\begin{definition}}\def\edefi{\end{definition}}
\newcommand{\IDEA}{\textbf{Idea of the Proof.} }
\newenvironment{idea}{\IDEA}{\hfill $\Box$}

\newcommand{\abs}[1]{\lvert#1\rvert}\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\absbig}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\absbigg}[1]{\biggl\lvert#1\biggr\rvert}
\newcommand{\absvar}[1]{\left\lvert#1\right\rvert}
\newcommand{\normvar}[1]{\left\lVert#1\right\rVert}
\renewcommand{\iff}{\quad\leftrightarrow\quad}
\newcommand{\huals}[1]{\begin{align}#1\end{align}}
\def\bmip{\begin{minipage}{\textwidth}}\def\emip{\end{minipage}}
\def\huga#1{\begin{gather} #1 \end{gather}}
\def\hugast#1{\begin{gather*} #1 \end{gather*}}
\def\hual#1{\begin{align} #1 \end{align}}
\def\hualst#1{\begin{align*} #1 \end{align*}}
\def\hueq#1{\begin{equation} #1 \end{equation}}
\def\hueqst#1{\begin{equation*} #1 \end{equation*}}

%%%%%%%%%%%%%%%%%%%%%% Hannes Def %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}\newcommand{\N}{{\mathbb N}}
\newcommand{\Q}{{\mathbb Q}}\newcommand{\Z}{{\mathbb Z}}

\def\CC{{\cal C}}\def\CK{{\cal K}}\def\CT{{\cal T}}\def\CU{{\cal U}}
\def\CV{{\cal V}}\def\CA{{\cal A}}\def\CE{{\cal E}}\def\CD{{\cal D}}  
\def\CF{{\cal F}}\def\CG{{\cal G}}\def\CH{{\cal H}}\def\CL{{\cal L}}
\def\CO{{\cal O}}\def\CP{{\cal P}}\def\CR{{\cal R}}\def\CS{{\cal S}}
\def\CM{{\cal M}}\def\CN{{\cal N}}\def\CZ{{\cal Z}}\def\CB{{\cal B}}
\def\CX{{\cal X}}\def\CY{{\cal Y}}
\def\OO{{\cal O}}\def\ee{{\rm e}}\def\e{{\rm e}}\def\ii{{\rm i}}
\def\setm{\setminus}\def\diag{{\rm diag}}\def\dist{{\rm dist}}
\def\spani{{\rm span}}\def\rmd{{\rm d}}\def\per{{\rm per}}
\def\unif{{\rm unif}}\def\Erf{{\rm Erf}}\def\erf{{\rm erf}}
\def\erfc{{\rm erfc}}
\def\spur{{\rm spur}}\def\vx{\vec x}
\def\pl{p_{\rm l}}\def\pnli{p_{\rm nl}^{\rm i}}\def\pnlm{p_{\rm nl}^{\rm m}}
\def\pnl{p_{\rm nl}}\def\cg{c_{\rm g}}
\def\uti{\tilde{u}}\def\vti{\tilde{v}}
\def\xt{\tilde{x}}\def\yt{\tilde{y}}

\def\ga{\gamma}\def\om{\omega}\def\th{\theta}\def\uh{\hat{u}}\def\vh{\hat{v}}
\def\noi{\noindent}\def\ds{\displaystyle}
\def\vt{\vartheta}\def\Id{\mbox{Id}}\def\pa{{\partial}}\def\lam{\lambda}
\newcommand{\bi}{\begin{itemize}}\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}\newcommand{\een}{\end{enumerate}}
\newcommand{\bce}{\begin{center}}\newcommand{\ece}{\end{center}}
\newcommand{\bci}{\begin{compactitem}}\newcommand{\eci}{\end{compactitem}}
\newcommand{\bcen}{\begin{compactenum}}\newcommand{\ecen}{\end{compactenum}}
\newcommand{\bcena}{\begin{compactenum}[(a)]}
\newcommand{\reff}[1]{(\ref{#1})}\newcommand{\ul}[1]{{\underline {#1}}}
\newcommand{\mbf}[1]{{\mathbf{#1}}}\newcommand{\ov}[1]{{\overline {#1}}}
%\newcommand{\ol}[1]{{\overline {#1}}}
\newcommand{\nonu}{\nonumber}
\newcommand{\spr}[1]{\left\langle #1 \right\rangle}
\newcommand{\hs}[1]{{\hspace{#1}}}\newcommand{\vs}[1]{{\vspace{#1}}}
\newcommand{\bhs}[1]{\mbox{\hspace{#1}}}
\def\eps{\varepsilon}\def\epsi{\epsilon}\def\aqui{\Leftrightarrow}
\def\ra{\rightarrow}\def\Ra{\Rightarrow}\def\la{\leftarrow}
\def\lra{\leftrightarrow}\def\lora{\longrightarrow}\def\loma{\longmapsto}
\newcommand{\barr}{\begin{array}}\newcommand{\earr}{\end{array}}
\newcommand{\bpm}{\begin{pmatrix}}\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bsm}{\left(\begin{smallmatrix}}
\newcommand{\esm}{\end{smallmatrix}\right)}
\newcommand{\ba}{\begin{array}}\newcommand{\ea}{\end{array}}
\def\dd{\, {\rm d}}\def\ri{{\rm i}}\def\sech{{\rm sech}}
\def\dx{\, {\rm d}x}\def\dds{\frac{\rm d}{{\rm d}s}}\def\rds{{\rm ds}}
\def\cc{{\rm c.c.}}\def\res{{\rm Res}}\def\er{{\rm e}}
\def\re{{\rm Re}}\def\im{{\rm Im}}\def\ccf{{\rm c.c.f}}
\def\spec{{\rm spec}}\def\om{\omega}\def\Om{\Omega}
\def\hot{{\rm h.o.t}}\def\ddt{\frac{\rm d}{{\rm d}t}}
\def\ddx{\frac{\rm d}{{\rm d}x}}\def\bphi{\varphi}\def\del{\delta}
\def\supp{{\rm supp}}\def\id{{\rm Id}}
\def\nab{\nabla}\def\eex{\hfill\mbox{$\rfloor$}}
\newcommand{\qedd}{\tag*{$\square$}}
\newcommand{\qeb}{\hfill\mbox{$\rfloor$}}
\DeclareMathOperator{\Res}{Res}\def\per{{\rm per}}\def\tw{\tilde w}
\def\sign{{\rm sign}}\def\Re{{\rm Re}}\def\Im{{\rm Im}}
\def\Del{\Delta}\def\na{\nabla}
\def\lamdtol{{\rm tol}_{\dot\lam}}\def\utt{{\tt u}}\def\Ftt{{\tt F}}
\def\phiti{\tilde{\phi}}\def\psiti{\tilde{\psi}}
\def\kti{\tilde{k}}\def\sig{\sigma}
\def\nag{\nabla{\gamma}}\def\lap{\Delta}\def\al{\alpha}
\def\fti{\tilde{f}}\def\gti{\tilde{g}}\def\wti{\tilde{w}}
\def\he{\hat{e}}\def\hemu{\hat{e}_{(\mu)}}\def\henu{\hat{e}_{(\nu)}}
\def\hemp{\hat{e}_{(\mu')}}\def\henp{\hat{e}_{(\nu')}}
\def\mup{{\mu'}}\def\nup{{\nu'}}
\def\wh{\widehat}\def\Ga{\Gamma}\def\Rti{\tilde{R}}\def\Lam{\Lambda}
\def\kap{\kappa}\def\Sig{\Sigma}
\def\rot{\nabla\times}\def\nati{\nabla\times}\def\nad{\nabla\cdot}

\def\xmin{{x_{\mbox{\small min}}}}\def\xmax{{x_{\mbox{\small max}}}} 
\def\un{u^{(0)}}\def\ue{u^{(1)}} \def\us{{\tilde{u}}}
\def\bd{\begin{displaymath}} \def\ed{\end{displaymath}}
\def\ba{\begin{array}} \def\ea{\end{array}}
\def\ua{u^{(1)}} \def\ub{u^{(2)}}\def\uta{u_t^{(1)}} \def\utb{u_t^{(2)}}
\def\eps{\varepsilon} \def\dt{\Delta t \;}
\def\lp{\Delta} \def\cd{(t,\cdot)}\def\cn{(0,\cdot)} \def\di{\displaystyle}
\def\xppaut{{\tt xppaut}}\def\xpp{{\tt xppaut}}
\def\matlab{{\tt matlab}}\def\oct{{\tt octave}}\def\uloc{\text{ul}}
\def\hurl{{\tt www.staff.uni-oldenburg.de/hannes.uecker/soft.html}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> p2pdef.tex <==
\def\pdep{{\tt pde2path}}\def\pdepo{{\tt pde2path}}
\def\PMAXP{Pontryagin's Maximum Principle}
\def\auto{{\tt AUTO}}\def\poc{{\tt p2poc}}
\def\p{\tt p} 
\def\oop{{\tt OOPDE}}\def\pocl{{\tt p2poclib}}
\def\holib{Hopf library}\def\mtom{{\tt mtom}}
\def\mlab{{\tt Matlab}}\def\ptool{{\tt pdetoolbox}}
\def\phome{{\tt www.staff.uni-oldenburg.de/hannes.uecker/pde2path}}
\def\dhome{/hh/path/pde2path/demos/acpbc}
\def\hdhome{/hh/path/pde2path/hopfdemos}
\def\Gbc{G_{\text{BC}}}\def\Qbc{Q_{\text{BC}}}


